Causal Analysis of Failures of Cyber-Physical Systems with Continuous Inputs

Modern autonomous Cyber-Physical Systems (CPSs), such as self-driving cars, operate in increasingly complex environments while expected to maintain high reliability. The black-box nature of many of these systems makes it impossible to fully verify their behavior prior to deployment. When a failure occurs, it is important to analyze it to guide improvements to system robustness. A recent work introduced the novel concept of leveraging the framework of actual causality for CPS failure explanation. However, that work considered only a discrete, binary causal model that cannot capture continuous changes in system inputs. In this paper, we address these limitations by extending the actual causality framework with the notion of distance to account for the continuous characteristics of the system. Specifically, we introduce the novel concepts of distance-weighted actual cause and distance-weighted degree of responsibility, enabling causal influence to account for the magnitude of changes required to avoid a failure, rather than only its cardinality. While motivated by the continuous nature of CPSs, this constitutes a general extension of the theory of actual causality and enables more fine-grained analysis of continuous inputs in any causal model. Building on these notions, we present an efficient, practical, system-agnostic explanation-derivation algorithm that uses distance-weighted responsibility to guide the explanation search. We experimentally evaluate our approach across a number of environments from two autonomous-driving simulators with black-box neural controllers. The results show that the proposed extension provides more effective guidance than the current discrete approach.

==> notes_from_meetings.tex <==
\section{KE notes from discussion 10/2}
Note that currently in the ICRA paper we defined our objective as finding necessity explanatinos, but then in the algorithm actually search for succicency. That was conflicting. We need to change the results/algorithm to reflect the correct objective.

Indeed, necessity explanations are more suitable for failures/"negative events", when we want something not to happen. These tell us what we need to change to avoid the failure from happening again.
Sufficiency explanatinos are for "positive events", when we want something to happen.

when deriving necessary events for collision, then we would always have the trivial explanation - of the object with which we collided. But we want to find if there are others, non-trivial explanations. This is sensible, especially if the object in collision is a part of the task definition, and cannot be removed. so we need to find "fixable causes".

I think explanations should be a variable subset that cannot be reduced. this is different than the absolute minimality requirement. It is less strict - it is like a local minimum. And I think it is indeed snesible that I will hvae a few explanatinos. Does this sit right with the definitions?

Our causal model has the same topology of the one from ICRA, but now the ranges of the variables = ranges of interventions are continuous and not binary (exists not exist)

This implies three theoretical extensions for this IROS paper:
(1) now the interventions we allow are continuous rather than binary
(2) now the responsibility needs to be based on the continuous distance between the samples.
(3) now the sampling distribution (of interventions, after the reponsibility ranking) should/may account for the distance; DK says we can, for example, do "binary search" for the best witness, based on distance (this is "algorithmic" sampling vs completely random sampling).


There are two layers of approximation when calculating the responsibility:
One is checking only some of the Actual Cause (AC) candidates (sampling subsets of the obstacles) [actually, not exactly, because AC should be a minimal subset].
Second is checking only some of the interventions possible for each candidate, to check if it is actually a cause or not (if I find one intervention that changes that outcome, then it is an actual cause) [previously we effectively checked only one intervention for each candidate].


\subsection{Algorithms for Tom [single context - the original failed run]:}

Responsibility Calculation, a two level sampling process:
User defined parameters: AC candidate sampling budget, intervention sampling budget per candidate

While in budget:
----Sample a subset X of the variables (observed obstacles) to be a candidate AC.
----While in budget:
--------Sample an intervention X' over X (i.e., scene perturbation)
--------If running the simulation with X' (all other vars not in X stay the same*) changes the outcome:
------------Measure distance d between the perturbed scene and the original scene
------------If the distance d is smaller than the distance observed thus far, save this simulation as X'\_best [this is the strongest witness for X being an AC/explanation].
// From this process we get a bunch of ACs and their strength. From this, we need to infer the variable responsibilities.
----For each variable (obstacle) o:
----// "summarize" its score from all the ACs in which it is involved
--------Calculate the average responsibility for o across all candidate ACs in which it was involved; the average should be weighted according to the strength/distance of each candidate AC's witness**

* this is enough here because we consider only a single context - the original scene.
**Tom, this is the formula you wrote. For now, just use the simpler one, which divides the responsibility equally among all obstacles that were involved (doesn't require extra distance calculation per variable). After that we can POTENTIALLY account for the the relative intervention size for that specific variable.
** this might be inconsistent with the definition of responsibility, as they take minimum in both summaries.

Explanation from responsibilities:
User defined parameters: thresholds for "substantial change", sampling budget per AC candidate

----Order all obstacles from high to low based on responsibilities
----AC = []
----For i from 0 ...
-------- AC = AC union \{xi\}
-------- // search for the smallest intervention on (all) the vars in AC that will change the outcome.
-------- If this AC was considred in the responsibility calculation process, then we have a witness for it (intervention that changes the outcome)-mark it as AC'; otherwise, sample until finding a witness for it (attempt within the sample budget for this AC, if couldn't find one after budget-move on).
-------- While remaining sampling budget: // try to improve the witness
-------- Sample an intervention of AC, mark it as AC''
-------- Calc the distance from the original, If the distance is smaller of AC': \\ check if this is a witness*
------------ Rerun the simulation with AC'', If outcome changes:
------------ Replace AC' with AC'', it is a better witness.
--------If the distance of AC' is smaller than A GIVEN THERHSHOLD D [marks the thershold of what changes is substantial enough]**
------------break
----Optionally: Try to reduce AC with an exhaustive search, like we have done before

* in the ICRA/discrete intervention case, it is easier - we dont need to check the distance. finding one witness is enough already. so we can skip the final optimization attempt of the witness.

** In the continuous case we HAVE TO define such a thershold, because the "exact goal" is zero-mesure, too small to find in the search. We have to expand it to a region. 


\hrule
* What was the summarization method in ICRA?

The algorithm we presented at ICRA contained only one level of sampling. But note that this was a specific case of the algorithm mentioned here, as the two sampling tiers collapsed into one, because of the discrete, binary interventions/distances in a depth-2 causal model. What we discuss here is the actual general algorithm/technique.

Another interesting point that came up after the meeting:
The original definition of actual cause takes into account minimality of the cause candidate (in terms of the number of variables). To account for the amount of change needed to change the outcome, it might be interesting to check minimality in terms of distance.
-- this was not a problem at icra because we had binary involvement for each variable (only a single possible intervention), so the only way to compare was by the number of variables involved.
single-context explanation = actual cause. Should remove the definition of actual cause. and discuss multi-context explanation in the journal version.

Need to define a measure for the quality of the explanation, accounting for both the number of vars and the size of change (distance).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> results_old.tex <==



\section{Experimental Evaluation (Old)}
\label{sec:evaluation-old}


\subsection{Results}

\Cref{tab:runs} and \Cref{fig:runs} report the mean computational effort, measured as the number of simulation runs required by each method compared to the exhaustive approach, which is exponential in the number of obstacles. Overall, the two distance-based methods substantially reduce the computational effort compared to the exhaustive search. They also generally achieve lower computational costs than the discrete setting, particularly in a higher number of obstacles. While no single method dominates across all settings, the simulation distance appears to be the most stable, requiring the lowest or the second lowest number of simulation runs in all settings. When comparing the sample budgets for the simulation distance, it generally performed better with 100 samples in a lower number of obstacles and with 200 samples in a higher number of obstacles.


\begin{table}[h]
\scriptsize
\centering
\setlength{\tabcolsep}{1pt}
\caption{Computational effort comparison. The mean amount of simulation runs required to find an explanation. Lower is better.}
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.0}
\begin{tabular}{c|| c c c c c c c}
\toprule
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\bfseries Discrete} & \multicolumn{2}{c}{\bfseries Simulation Distance} & \multicolumn{2}{c}{\bfseries Euclidean Distance}  \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
\bfseries \#Obs & \bfseries Exhaustive &  
\bfseries 100 samp. & \bfseries 200 samp. & \bfseries 100 samp. & \bfseries 200 samp. & \bfseries 100 samp. & \bfseries 200 samp.  \\
\midrule
10 & 1024 & 911 & 995 & \bfseries726 & 794 & 847 & 943 \\
11 & 2048 & 1488 & 1338 & 953 & 1263 & \bfseries697 & 1105 \\
12 & 4096 & 2329 & 2677 & 2445 & \bfseries1625 & 2361 & 3581 \\
13 & 8192 & 5750 & 6194 & 2593 & 3313 & \bfseries2420 & 2605 \\
14 & 16384 & 10694 & 10766 & 7244 & \bfseries5975 & 8105 & 9266 \\
\bottomrule
\end{tabular}
\label{tab:runs}
\end{table}

% \begin{figure}[h]
%     \begin{tikzpicture}[scale=0.93, transform shape]
%     \pgfplotsset{%
%     width=0.5\textwidth,
%     height=0.35\textwidth
%     }
% \begin{axis}[
%     % width=0.84\linewidth,
%     % height=0.62\linewidth,
%     xlabel={Obstacles},
%     ylabel={Simulation runs},
%     % xmin=5.5, xmax=15.5,
%     xtick={10,11,12,13,14},
%     ytick={0,5000,10000,15000},
%     scaled ticks=false,
%     ymajorgrids,
%     grid style={gray!20},
%     legend style={
%       at={(rel axis cs:0.05,0.97)},
%       anchor=north west,
%       draw=none,
%       fill=white, fill opacity=0.85,
%       rounded corners=2pt,
%       font=\scriptsize,
%       % row sep=1.6pt,
%       % column sep=4pt,
%       nodes={inner sep=1pt, text depth=0.15ex}
%     },
%     legend image code/.code={
%         \draw[#1, line width=1.2pt] (0cm,0cm) -- (0.3cm,0cm);
%     },
%     % legend image post style={xscale=0.25, yscale=0.25},
%     tick style={black!60},
%     tick label style={/pgf/number format/fixed},
%     every axis plot/.append style={thick},
% ]

% % CSV with headers:
% % obstacles,rg100,rg200,rg300,rgo100,rgo200,rgo300,es
% \pgfplotstableread[col sep=comma]{results/runs_results.csv}\datatable

% \addplot[color=black!70] table[x=obstacles, y=exhaustive] {\datatable};
% \addlegendentry{Exhaustive search}

% \addplot[color=red!50] table[x=obstacles, y=discrete_100] {\datatable};
% \addlegendentry{Discrete 100 samples}

% \addplot[color=red!100] table[x=obstacles, y=discrete_200] {\datatable};
% \addlegendentry{Discrete 200 samples}

% \addplot[color=green!50] table[x=obstacles, y=euclidean_100] {\datatable};
% \addlegendentry{Euclidean 100 samples}

% \addplot[color=green!100] table[x=obstacles, y=euclidean_200] {\datatable};
% \addlegendentry{Euclidean 200 samples}

% \addplot[color=blue!50] table[x=obstacles, y=distance_100] {\datatable};
% \addlegendentry{Simulation 100 samples}

% \addplot[color=blue!100] table[x=obstacles, y=distance_200] {\datatable};
% \addlegendentry{Simulation 200 samples}



% \end{axis}
% \end{tikzpicture}
%     \caption{The mean computational effort (simulation runs) required by each method. Lower is better.}
%     \label{fig:runs}
% \end{figure}



\Cref{tab:explanation-size-success-rate} reports the percentage of minimal explanations obtained by each method, measured by comparing the size of the generated explanation to that returned by exhaustive search. Overall, the discrete variant demonstrates high performance, reaching minimal explanations in nearly all settings. The distance-based methods exhibit slightly lower minimality rates, although their performance does not appear to deteriorate as the number of obstacles increases. To complement this analysis, \Cref{tab:explanation-size-non-minimal} presents the mean deviation from minimality for the cases in which the methods failed to produce a minimal explanation. These measurements are computed only over falsifying examples where the explanation was non-minimal; accordingly, results are shown only for configurations whose success rate in \Cref{tab:explanation-size-success-rate} is below 100\%. Overall, even when the explanations are not minimal, the deviation is small. In most cases, the generated explanation exceeds the minimal one by only a single obstacle, indicating that the methods remain close to optimal if not optimal.

\begin{table}[h]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\caption{Optimality of explanation, measured as the percentage of cases for which the generated explanation is minimal (that is, equal in size to the one obtained by exhaustive search). Higher is better.}
\begin{tabular}{c|| c c c c c c}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\bfseries Discrete} & \multicolumn{2}{c}{\bfseries Simulation Distance} & \multicolumn{2}{c}{\bfseries Euclidean Distance} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\bfseries \#Obs &
\bfseries 100 samp. & \bfseries 200 samp. & \bfseries 100 samp. & \bfseries 200 samp. & \bfseries 100 samp. & \bfseries 200 samp.  \\
\midrule
10 & 100\% & 100\% & 95\% & 90\% & 95\% & 95\% \\
11 & 100\% & 95\% & 100\% & 95\% & 90\% & 95\% \\
12 & 100\% & 95\% & 95\% & 85\% & 100\% & 100\%  \\
13 & 100\% & 100\% & 80\% & 90\% & 80\% & 70\% \\
14 & 100\% & 100\% & 95\% & 90\% & 100\% & 90\% \\
\bottomrule
\end{tabular}
\label{tab:explanation-size-success-rate}
\end{table}

\begin{table}[h]
\scriptsize
\centering
\setlength{\tabcolsep}{3pt}
\caption{Magnitude of sub-optimality, measured as the mean size-difference between the generated explanation and the minimal explanation (obtained by exhaustive search). Values only shown for cases where the success rate in \autoref{tab:explanation-size-success-rate} is below 100\%. Lower is better.}
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.0}
\begin{tabular}{c|| c c c c c c}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\bfseries Discrete} & \multicolumn{2}{c}{\bfseries Simulation Distance} & \multicolumn{2}{c}{\bfseries Euclidean Distance}  \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\bfseries \#Obs &
\bfseries 100 samp. & \bfseries 200 samp. & \bfseries 100 samp. & \bfseries 200 samp. & \bfseries 100 samp. & \bfseries 200 samp.  \\
\midrule
10 & - & - & 1.0 & 1.0 & 1.0 & 1.0 \\ 
11 & - & 1.0 & - & 2.0 & 1.0 & 1.0 \\ 
12 & - & 1.0 & 1.0 & 1.0 & 1.0 & -  \\
13 & - & - & 1.0 & 1.0 & 1.0 & 1.0 \\
14 & - & - & 1.0 & 1.5 & - & 2.0 \\
\bottomrule
\end{tabular}
\label{tab:explanation-size-non-minimal}
\end{table}

Overall, the results demonstrate a tradeoff between explanation minimality and computational effort. Incorporating the simulation-distance approach substantially improves scalability, reducing the number of simulation runs while maintaining near-minimal explanations, and thus offering a stable balance between optimality and computational effort.




==> runs_plot_old.tex <==
\begin{figure}[ht]
    \begin{tikzpicture}[scale=0.9, transform shape]
    \pgfplotsset{%
    width=0.5\textwidth,
    height=0.3\textwidth
    }
\begin{axis}[
    % width=0.84\linewidth,
    % height=0.62\linewidth,
    xlabel={Obstacles},
    ylabel={Simulation runs},
    % xmin=5.5, xmax=15.5,
    xtick={10,11,12,13,14},
    ytick={0,5000,10000,15000},
    scaled ticks=false,
    ymajorgrids,
    grid style={gray!20},
    legend style={
      at={(rel axis cs:0.05,0.97)},
      anchor=north west,
      draw=none,
      fill=white, fill opacity=0.85,
      rounded corners=2pt,
      font=\scriptsize,
      % row sep=1.6pt,
      % column sep=4pt,
      nodes={inner sep=1pt, text depth=0.15ex}
    },
    legend image code/.code={
        \draw[#1, line width=1.2pt] (0cm,0cm) -- (0.3cm,0cm);
    },
    % legend image post style={xscale=0.25, yscale=0.25},
    tick style={black!60},
    tick label style={/pgf/number format/fixed},
    every axis plot/.append style={thick},
]

% CSV with headers:
% obstacles,rg100,rg200,rg300,rgo100,rgo200,rgo300,es
\pgfplotstableread[col sep=comma]{results/runs_results.csv}\datatable

\addplot[color=red!70] table[x=obstacles, y=exhaustive] {\datatable};
\addlegendentry{exhaustive}

\addplot[color=green!50] table[x=obstacles, y=discrete_100] {\datatable};
\addlegendentry{discrete 100 samples}

\addplot[color=green!100] table[x=obstacles, y=discrete_200] {\datatable};
\addlegendentry{discrete 200 samples}

\addplot[color=blue!50] table[x=obstacles, y=distance_100] {\datatable};
\addlegendentry{distance 100 samples}

\addplot[color=blue!100] table[x=obstacles, y=distance_200] {\datatable};
\addlegendentry{distance 200 samples}



\end{axis}
\end{tikzpicture}
    \caption{The mean computational effort (simulation runs) required by each method.}
    \label{fig:runs}
\end{figure}

